A Few-Shot Semantic Parser for Wizard-of-Oz Dialogues with the Precise ThingTalk Representation

Previous attempts to build effective semantic parsers for Wizard-of-Oz (WOZ) conversations suffer from the difficulty in acquiring a high-quality, manually annotated training set. Approaches based only on dialogue synthesis are insufficient, as dialogues generated from state-machine based models are poor approximations of real-life conversations. Furthermore, previously proposed dialogue state representations are ambiguous and lack the precision necessary for building an effective agent. This paper proposes a new dialogue representation and a sample-efficient methodology that can predict precise dialogue states in WOZ conversations. We extended the ThingTalk representation to capture all information an agent needs to respond properly. Our training strategy is sample-efficient: we combine (1) fewshot data sparsely sampling the full dialogue space and (2) synthesized data covering a subset space of dialogues generated by a succinct state-based dialogue model. The completeness of the extended ThingTalk language is demonstrated with a fully operational agent, which is also used in training data synthesis. We demonstrate the effectiveness of our methodology on MultiWOZ 3.0, a reannotation of the MultiWOZ 2.1 dataset in ThingTalk. ThingTalk can represent 98% of the test turns, while the simulator can emulate 85% of the validation set. We train a contextual semantic parser using our strategy, and obtain 79% turn-by-turn exact match accuracy on the reannotated test set.

==> intro-old.tex <==
\section{Introduction}

Virtual assistants and task-oriented conversational agents are poised to transform how consumers interact with computers. Alexa has over 100,000 skills, and we envision many more websites will integrate ``chatbot'' capabilities in the near future.

Commonly, commercial conversational agents are built using a modular design~\tocite: a \textit{dialogue state tracking} (DST) component understands the user input and the state of the dialogue up to a point, a \textit{dialogue policy} component decides the high-level action the agent should perform, and a \textit{natural language generation} (NLG) component that produces the actual reply to the user. The modular approach has the advantage that the dialogue policy can be programmed, rather than learned end-to-end from data~\tocite); hence, the agent is more reliable, more interpretable, and can encode business-specific behavior rules.

In a modular design, the quality of the conversational agent depends heavily on the dialogue state tracking. Rule-based state tracking approaches, based on dialogue trees and intent classifiers, tend to be brittle in the face of unexpected dialogue flows. Previous work~\tocite has proposed used end-to-end neural DST, in which a neural network is trained on a full dialogue to predict the state of the dialogue at all turns. While end-to-end DST can be very effective, it relies on very large datasets of dialogues, which must be annotated with a formal representation at every turn.

As a way to acquire dialogue data for DST, previous work has proposed the \textit{wizard-of-oz} technique, in which two human crowdworkers are asked to converse simulating the interaction with the conversational agent, and annotate each turn as they proceed. This makes WOZ datasets are very expensive to acquire. The largest such dataset is MultiWOZ~\cite{budzianowski2018large}, a dataset of XXX dialogues in 5 transactional domains. Additionally, WOZ datasets suffer from poor annotation quality. MultiWOZ has been fully reannotated once~\cite{eric2019multiwoz}, but still has significant errors and inconsistencies in the annotations~\cite{zhou2019multi}. Finally, because WOZ datasets are human-human conversations, they do not match the behavior of the dialogue agent at inference time, and neural DST trained on such datasets must understand dialogues that cannot occur in practice.

Can we retain the rule-based interpretability of a modular conversational agent design, and the flexibility of a neural DST solution, while solving the challenges of acquiring training data? We hypothesis that much of the complexity of DST comes from the use of human-human dialogues as training. We propose instead to build a DST based exclusively on \textit{synthesized} dialogues constructed based on the \textit{conversational model} of how the user and the agent interact. The same model can be employed at test time to define the dialogue policy, removing any impossible dialogue flows from the DST training. As the dialogues are synthesized, they are automatically annotated, and the annotation is correct by construction. Finally, because we can annotate the agent side in addition to the user, a DST model in this framework needs not learn how interpret the agent utterances.

Specifically, in our new methodology, we propose:
\begin{enumerate}
\item Representing the dialogue between the user and the agent in  \textit{conversational model}. A conversational model is a kind of dialogue state machine that contains the information to express the utterances in the dialogue (in the form of \textit{templates}) with their precise formal representation. The formal representation is a \textit{domain specific language} (DSL) designed to capture all the information necessary to continue the dialogue, both at training and at test time. It is a superset of previous approaches that only tracked slot values.
\item Using synthesis to quickly and cheaply obtain large training sets of dialogues. These dialogues are annotated at every turn with the exact, formal state of the conversation, which includes all the actions and API calls that the agent has made up to that point.
\item Training a neural network that, given the formal state of the conversation before the user speaks, and the current user utterance, predicts the next state of the conversation. The network is trained turn by turn, so it can understand long conversations without exponentially many training samples. It is trained exclusively on user natural language, eliminating a source of confusion in training. We have developed a novel neural architecture, called \ctxnlu (Contextual Natural Language Understanding), that can perform well on this task. \ctxnlu is based on sequence-to-sequence~\cite{sutskever2014sequence} and the BERT encoder~\cite{devlin2018bert}. 
\item Using a small amount of manually annotated human-human dialogue data for evaluation. Because the amount is small, the annotation can be performed by a developer of the conversational agent, and can be made to match the conversational model exactly, removing any ambiguity in the annotation specification. If the conversational model can express all or most flows in the annotated data, and the neural DST achieves high accuracy on it, we can be confident that, at test time, the conversational agent will understand the user and imitate a skilled human agent.
\end{enumerate}

Using a conversational agent for task-oriented dialogues was previously proposed by \newcite{zeroshotmultiwoz}, which used a simple dialogue state machine and synthesis to augment the MultiWOZ dataset for zero-shot learning. The previous work mixed human-human conversations with synthesized conversation. In this paper, we take that work to the logical conclusion, by eliminating all human agents from the training data, thus cutting the complexity of DST in half, and enabling the neural network to work turn-by-turn instead of a conversation at a time.

We build upon the previously proposed dialogue state machine to build a full conversational model for \textit{transaction dialogues}, an important family of task-oriented dialogues in which the user is interested in performing an action using some object in a database accessible by the agent. Transaction dialogues cover the 5 domains in the MultiWOZ datasets, as well as many use cases for task-oriented conversational agents in practice. The DSL in our conversational model is based on ThingTalk with database extensions~\cite{geniepldi19, xu2020schema2qa} \TODO{GC: I'm not sure how much we need to talk about ThingTalk - we could say the representation includes slots which are either requested, proposed, or accepted and that would cover 99\% of the dev set}. Usign a programming language with known semantics eliminates any ambiguity in annotating the dev and test sets. Furthemore, we can decouple the domain-specific execution aspects of the agent behavior from the general notion of continuing the transaction. Hence, our conversational model is \textit{domain-independent}: by specifying the database schema, the API calls, and small natural language annotations for both, the conversational model can be used to build an agent for a new domain.

We have applied our methodology and conversational model to the well-known MultiWOZ setting~\cite{budzianowski2018large}. To evaluate our approach, we re-annotated the dev and test sets using our language. This manual annotation solves many of the problems that were present in the 2.1 version of the dataset. It includes the new information necessary to undersand the user utterances: the agent dialogue act, any slot proposed by the agent, and the result of querying the data. The reannotated data can also be used to evaluate standard DST models trained on full sentences. We will release the reannotated data upon publication; a sample is included in the supplementary materials.

\subsection{Contributions}

The contribution of our paper are the following:
\begin{itemize}
\item A new methodology for building task-oriented conversational agents, based on formal languages and data synthesis.
\item The \ctxnlu neural model for dialogue state tracking, that incorporates the current formal state of the dialogue and produces the new state. Our model is the first neural DST model that need not learn how to interpret agent sentences.
\item A novel conversational model for transaction dialogues. The model captures many realistic flows between the user and the agent, and allows to build an agent that can mimic human-level understanding and human behavior.
\item Experimental results show that our approach can achieve high accuracy on the MultiWOZ dataset, without using any human-written training data.
\end{itemize}
